Fine-tuning CNN Image Retrieval with No Human Annotation

Image descriptors based on activations of Convolutional Neural Networks (CNNs) have become dominant in image retrieval due to their discriminative power, compactness of representation, and search efficiency. Training of CNNs, either from scratch or fine-tuning, requires a large amount of annotated data, where a high quality of annotation is often crucial. In this work, we propose to fine-tune CNNs for image retrieval on a large collection of unordered images in a fully automated manner. Reconstructed 3D models obtained by the state-of-the-art retrieval and structure-from-motion methods guide the selection of the training data. We show that both hard-positive and hard-negative examples, selected by exploiting the geometry and the camera positions available from the 3D models, enhance the performance of particular-object retrieval. CNN descriptor whitening discriminatively learned from the same training data outperforms commonly used PCA whitening. We propose a novel trainable Generalized-Mean (GeM) pooling layer that generalizes max and average pooling and show that it boosts retrieval performance. Applying the proposed method to the VGG network achieves state-of-the-art performance on the standard benchmarks: Oxford Buildings, Paris, and Holidays datasets.

==> ext-plots.tex <==
\usepackage{tikzextern}
%\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> fig_holidays_query_sample.tex <==
\begin{figure*}[t]
\begin{center}
\foreach \q in {1,...,40}
{\includegraphics[height=1.03cm]{fig/holidays_query_sample/q\q.jpg} \hspace{-1pt}}%
\end{center}
\caption{Holidays dataset: example queries. The dataset contains, not only buildings and landmarks, but also a large number of natural landscapes, indoor scenes and everyday planar or 3D objects.\label{fig:holidays}}%
\end{figure*}

==> fig_matches.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t!]
%
\begin{center}
\def\queryone{42}
\def\dbimageone{211}
%
\foreach \p in {1,...,5}{
\begin{tabular}{@{\sssp}c@{\sssp}c@{\ssp}c@{\bsp}c@{\ssp}c@{\bsp}c@{\ssp}c}
\raisebox{-23pt}{\hspace{-20pt}\def\col{p\p}\input{fig_gemp_vs_alpha}\hspace{-5pt}}&
\includegraphics[height=80pt]{fig/heatmaps/q\queryone_db\dbimageone_net1_p\p_al1_1}  &
\includegraphics[height=80pt]{fig/heatmaps/q\queryone_db\dbimageone_net1_p\p_al1_2}  &
\includegraphics[height=80pt]{fig/heatmaps/q\queryone_db\dbimageone_net1_p\p_al3_1}  &
\includegraphics[height=80pt]{fig/heatmaps/q\queryone_db\dbimageone_net1_p\p_al3_2}  &
\includegraphics[height=80pt]{fig/heatmaps/q\queryone_db\dbimageone_net1_p\p_al10_1} &
\includegraphics[height=80pt]{fig/heatmaps/q\queryone_db\dbimageone_net1_p\p_al10_2}\\
\end{tabular}
}
\end{center}
\vspace{-20pt}
\hspace{155pt}$p = 1$\hspace{115pt}$p = 3$\hspace{115pt}$p = 10$
\caption{Visualization of the CNN responses $\cX_{k}$ raised to the power of $p$ which are projected on the original image for several feature maps and for different values of $p$. 
We show the case for $p=1$ which corresponds to SPoC and the case for larger values of $p$  as in GeMP before the summation of (\ref{equ:gemp}). 
The selected feature maps are the ones that correspond to the SPoC vector ($p=1$) components that have the highest contribution to the pairwise image similarity. We show one feature map per row.
On the left we show the ratio $\nicefrac{\f^{(g)}_k}{\f^{(m)}_k}$ versus various values of $p$ (figure derived for the right image of the pair).
Examples shown use the off-the-shelf VGG.\label{fig:sump_matches}}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> fig_matches_ft1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t!]
%
\begin{center}
\def\queryone{11}
\def\dbimageone{2}
%
\begin{tabular}{c@{\hspace{10pt}}c@{\hspace{20pt}}c@{\hspace{10pt}}c@{\hspace{20pt}}c@{\hspace{10pt}}c}
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p1_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p1_al2_9_2}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p2_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p2_al2_9_2}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p3_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p3_al2_9_2}  \\
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p4_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p4_al2_9_2}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p5_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p5_al2_9_2}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p6_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p6_al2_9_2}  \\
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p7_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p7_al2_9_2}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p8_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p8_al2_9_2}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p9_al2_9_1}  &
\includegraphics[height=70pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p9_al2_9_2}  \\

\end{tabular}
\end{center}
\caption{Caption}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t!]
%
\begin{center}
\def\queryone{32}
\def\dbimageone{5}
%
\begin{tabular}{c@{\hspace{10pt}}c@{\hspace{20pt}}c@{\hspace{10pt}}c@{\hspace{20pt}}c@{\hspace{10pt}}c}
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p1_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p1_al2_9_2}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p2_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p2_al2_9_2}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p3_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p3_al2_9_2}  \\
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p4_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p4_al2_9_2}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p5_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p5_al2_9_2}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p6_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p6_al2_9_2}  \\
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p7_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p7_al2_9_2}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p8_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p8_al2_9_2}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p9_al2_9_1}  &
\includegraphics[height=50pt]{fig/heatmaps_n/q\queryone_db\dbimageone_p9_al2_9_2}  \\

\end{tabular}
\end{center}
\caption{Caption}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> no-plots.tex <==
\newcommand{\extfig}[2]{!}
\newcommand{\extdata}[1]{}


==> tab_exp_stateofart_BoW.tex <==
\begin{table*}[t!]
\newcommand{\ebA}{\texttt{\bf{A}}}
\newcommand{\ebV}{\texttt{\bf{V}}}
% \newcommand{\ebf}{\texttt{\bf{f}}}
\newcommand{\ebf}{{\scriptsize{$\blacksquare$}}}
\newcommand{\our}{$\boldsymbol{\star}$\xspace}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\def\arraystretch{1.3}%  1 is the default, row height
\newcommand\cw{1.8cm}
% \centering
\caption{Performance comparison with the state of the art methods that use re-ranking (R) and query expansion (QE). F-tuned: Use of the fine-tuned network (yes), or the off-the-shelf network~(no), not applicable for the methods using local features (n/a). Dim:~Dimensionality of the final compact image representation, not applicable (n/a) for the BoW based methods due to the sparse representation and use of the inverted file. Our methods are marked with \our and they are always accompanied by multi-scale and \cpl2. Previous state of the art highlighted in \protect\ob{bold}, new state of the art in \protect\nb{red outline}. Best viewed in color.
\label{tab:stateofartBoW}}
% \vspace{-5pt}
% \footnotesize
\begin{center}
\setlength{\tabcolsep}{0.2mm}
\begin{tabular}{|C{1cm}|@{~~}L{4cm}|C{1.2cm}|C{1cm}|C{\cw}|C{\cw}|C{\cw}|C{\cw}|C{\cw}|}
    \hline
    Net & Method & F-tuned & Dim & 
    Oxford5k & Oxford105k & Paris6k & Paris106k & Holidays \\ 
    \hline\hline
    \multirow{3}{*}{n/a} 
    & BoW~(1M)~+~R~+~QE~\cite{CMPM11} & n/a & n/a & 82.7 & 76.7 & 80.5 & 71.0 & -- \\
    & BoW~(16M)~+~R~+~QE~\cite{MPCM13} & n/a & n/a & 84.9 & 79.5 & 82.4 & 77.3 & 75.8 \\
    & HQE~(65k)~\cite{TJ14} & n/a & n/a & 88.0 & 84.0 & 82.8 & -- & -- \\
    \hline
    \multirow{5}{*}{VGG} 
    & CroW~+~QE~\cite{KMO15} & no & 512 & 72.2 & 67.8 & 85.5 & 79.7 & -- \\
    & R-MAC~+~R~+~QE~\cite{TSJ16} & no & 512 & 77.3 & 73.2 & 86.5 & 79.8 & -- \\ 
    & BoW-CNN~(25k)~+~R~+~QE~\cite{MMOS+16} & no & n/a & 78.8 & 65.1 & 84.8 & 64.1 & -- \\
    & R-MAC~+~QE~\cite{GARL16} & yes & 512 & \ob{89.1} & \ob{87.3} & \ob{91.2} & \ob{86.8} & -- \\
%     \our MAC+R+QE & \ebf & 512 & 85.0 & 81.8 & 86.5 & 78.8 & -- & -- \\
%     \our R-MAC+R+QE & \ebf & 512 & 82.9 & 77.9 & 85.6 & 78.3 & -- & -- \\
    & \our GeMP~+~QE & yes & 512 & \nb{90.7} & \nb{88.6} & \nb{92.2} & \nb{88.0} & {~~}\nb{89.2}$^\dagger$ \\
    \hline
\end{tabular}
\end{center}
% \vspace{-5pt}
\scriptsize
$~~~~~~~~~~~~~~~~~^\dagger$:~We do not perform QE on Holidays as it is not a standard practice.
\end{table*} 
